Charged Black Holes with Yukawa Potential

This study derives a novel family of charged black hole solutions featuring short- and long-range modifications. These ones are achieved through a Yukawa-like gravitational potential modification and a nonsingular electric potential incorporation. The short-range corrections encode quantum gravity effects, while the long-range adjustments simulate gravitational effects akin to those attributed to dark matter. Our investigation reveals that the total mass of the black hole undergoes corrections owing to the apparent presence of dark matter mass and the self-adjusted electric charge mass. Two distinct solutions are discussed: a regular black hole solution characterizing small black holes, where quantum effects play a crucial role, and a second solution portraying large black holes at considerable distances, where the significance of Yukawa corrections comes into play. Notably, these long-range corrections contribute to an increase in the total mass and hold particular interest as they can emulate the role of dark matter. Finally, we explore the phenomenological aspects of the black hole. Specifically, we examine the influence of electric charge and Yukawa parameters on thermodynamic quantities, the quasinormal modes for the charged scalar perturbations as well as for the vector perturbations, analysis of the geodesics of light/massive particles, and the accretion of matter onto the charged black hole solution.

==> Scalar.tex <==
% Scalar perturbations stuff removed from our original paper

\subsection{Charged scalar perturbations}
This section will closely follow the discourse presented in \cite{Cuadros-Melgar:2021sjy}. Our focus will be on analyzing a perturbation of a charged scalar field denoted as $\Psi$, which can be described by the Klein-Gordon equation
\begin{equation}\label{kge}
[(\nabla^\nu - iqA^\nu)(\nabla_\nu -iqA_\nu) -\mu^2] \Psi =0.
\end{equation}
Here, the parameters $\mu$ and $q$ represent the mass and charge of the field $\Psi$, respectively, while the electromagnetic potential $A_\mu = (-\mathcal{Q}/\sqrt{r^2+l_0^2}, 0, 0, 0)$ characterizes the BH. To simplify, we will consider the limit $l_0/r \to 0$, leading to $A_\mu = (-\mathcal{Q}/r, 0, 0, 0)$. Throughout our discussion, we will employ the background geometry described by Eq. \eqref{metric16}, resulting in a spherically symmetric metric as per Eq. \eqref{metric16}. The perturbed scalar field is denoted by $\Psi(t, r, \theta, \phi) = e^{-i\omega t} R(r) e^{im\phi} S(\theta)$, where $S(\theta) = P_\ell^m(\cos\theta)$ represents the associated Legendre polynomials. Consequently, the radial component of Eq. \eqref{kge} takes the form,  
\begin{eqnarray}
\label{feq1}
&&f^2 \frac{d^2 R}{dr^2} + \left(\frac{2f^2}{r} + ff' \right)
\frac{dR}{dr} \\\notag
&+& \left[\omega^2 + 
2q\omega \Phi + q^2 \Phi^2-\mu^2 f - \ell (\ell
+1)\frac{f}{r^2}\right] R = 0. 
\end{eqnarray}
One can define $\Delta_r = r^2 \, f(r)$ then by including the BH charge; we can rewrite the last equation as
\begin{eqnarray}\label{radial}
&&\Delta_r \frac{d}{dr}\left(\Delta_r \frac{dR}{dr}\right) \\\notag
&+& \left\{
(\omega r^2 -q \mathcal{Q} r)^2 - \Delta_r \left[\ell (\ell +1) + \mu^2 r^2\right]
\right\} R = 0. 
\end{eqnarray}
Furthermore, in terms of the tortoise coordinate defined as $dr_* = dr/f(r),  $
along with $R(r) =X(r)/r$, Eq. \eqref{radial} reads
\begin{equation}\label{Xeq}
\frac{d^2 X}{dr_*^2} + \mathcal{V} \, X = 0,  
\end{equation}
where the potential can be written as \cite{Cuadros-Melgar:2021sjy}
\begin{equation}\label{pot}
\mathcal{V} = \left( \omega - \frac{q \mathcal{Q}}{r} \right)^2 - f(r)
\left[ \frac{\ell (\ell +1)}{r^2} + \mu^2 + \frac{f'(r)
    }{r}  \right]. 
\end{equation}
Let us check the scalar field behavior near the horizons. Near the
event horizon $r\rightarrow r_+$ we have $f(r_+)\rightarrow 0$ and from Eq. \eqref{pot} we see that \cite{Cuadros-Melgar:2021sjy}
\begin{equation}
\mathcal{V} \rightarrow \left( \omega - \frac{q \mathcal{Q}}{r_h}\right) ^2 = (\omega
+q\Phi_h)^2. 
\end{equation}
Thus, the scalar field behaves as 
$e^{-i\omega t \pm i (\omega+q\Phi_h) r_*}$ with $\Phi_h$ being the
electromagnetic potential at the event horizon. Moreover, as there are only
ingoing waves at the horizon (classically, nothing comes out from
  $r_h$), we should choose the ($-$) sign. 
 \subsubsection*{The WKB approximation} 
In this case the potential \eqref{pot} in terms of $f(r)$ can be
approximated as 
\begin{equation}\label{newpot}
\mathcal{V}  (r) \approx \left(\omega - \frac{q \mathcal{Q}}{r}\right)^2 - \mu^2 f(r). 
\end{equation}
So that we can use the WKB approximation to
extract the frequencies through the following equation,  
\begin{equation}\label{schutz}
\frac{i\,  \mathcal{V}(r_* ^o)}{\sqrt{2\,  \mathcal{V}''(r_* ^o)}} = n+\frac{1}{2}\,  ; \quad n=0,  1,  2,  ...
\end{equation}
where $\mathcal{V}''=\frac{d^2 \mathcal{V}}{dr_* ^2}$ and $r_* ^o $ or $(r_* ^o\equiv r_0)$ is the extremum
point where $\mathcal{V}'(r_* ^o)=0$, which yields
\begin{equation}\label{om1}
\omega - \frac{q \mathcal{Q}}{r_0} = \frac{\mu^2 f'(r_* ^o) r_0 ^2}{2q \mathcal{Q} f(r_* ^o)}\,  .
\end{equation}
In this expression, once more, a prime ($'$) denotes a derivative with respect to the tortoise coordinate. By expressing $\omega$ as $\omega = \omega_R - i \omega_I$, we can facilitate the decoupling of the real part, wherein
\begin{equation}\label{om2}
\left(\omega_R - \frac{q \mathcal{Q}}{r_0}\right)^2 - \mu^2 f(r_* ^o) = 0,  
\end{equation}
Finally, it can be shown that for the real part of the near-extremal frequency, one can obtain 
\begin{equation}\label{hodf}
\omega_{R} \approx \frac{q \mathcal{Q}}{r_+} \pm \frac{\sqrt{2} \,  \mu \kappa_+
  r_+}{\sqrt{1-3(\mathcal{Q}/r_+)^2 + 2(qQ/\mu r_+)^2}}\,  .
\end{equation}
In order to obtain a better compression of Eq. (\ref{hodf}) to the reader, we plot Fig. \ref{wr}. Here, we notice that as $r_{+}$ increases, $\omega_{R}$ strongly decreases. 


\begin{figure}
    \centering
    \includegraphics[scale=0.45]{wr.pdf}
    \caption{Different values of $\omega_{R}$ are shown as a function of $r_{+}$.}
    \label{wr}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Massless scalar perturbations}

In our computations, we examine perturbations utilizing the scalar field. Accordingly, we formulate the Klein–Gordon equation within the framework of a curved spacetime
\ie
\frac{1}{\sqrt{-g}}\partial_{\mu}(g^{\mu\nu}\sqrt{-g}\partial_{\nu}\Phi) = 0.\label{KL}
\fe
While exploring the captivating realm of \textit{backreaction} effects in this particular scenario, it is essential to note that this manuscript refrains from an in-depth examination of this aspect. Instead, our emphasis is directed towards the exploration of other facets. The primary focus is to study the scalar field comprehensively as a small perturbation. Furthermore, leveraging the spherical symmetry inherent in the system, we seize the opportunity to decompose the scalar field in a specific manner, as elucidated below:
\ie
\Phi(t,  r,  \theta,  \varphi) = \sum^{\infty}_{l=0}\sum^{l}_{m=-l}r^{-1}\Psi_{lm}(t,  r)Y_{lm}(\theta,  \varphi),  \label{decomposition}
\fe
By representing the spherical harmonics as $Y_{lm}(\theta, \varphi)$, we can introduce the decomposition of the scalar field as outlined in Eq. \eqref{decomposition} into Eq. \eqref{KL}. This substitution transforms the equation into a Schrödinger--like form, imbuing it with wave-like properties that make it amenable to our analytical scrutiny
\ie
-\frac{\partial^{2} \Psi}{\partial t^{2}}+\frac{\partial^{2} \Psi}{\partial r^{*2}} + V_{eff}(r^{*})\Psi = 0.\label{schordingereq}
\fe
The potential $V_{eff}$, widely recognized as the \textit{Regge--Wheeler} potential or the effective potential, serves as a repository of crucial information concerning the BH's geometry. Additionally, we introduce the tortoise coordinate $r^{*}$, spanning the entirety of spacetime as $r^{*}\rightarrow \pm \infty$. Following a series of algebraic manipulations, we can articulate the effective potential explicitly as
\ie
\begin{split}
& V_{eff}(r) = \\
& f(r) \left( \frac{l (l+1)}{r^2}+\frac{-\frac{2 \mathcal{Q}}{r^3}+\frac{2 \mathcal{M}}{r^2}-\frac{2 \Lambda  r}{3}+\frac{\mathcal{M}_{\alpha}}{(\alpha +1) \lambda ^2}}{r} \right).
\end{split}
\fe

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsubsection*{The WKB approximation}



Within this section, our objective is to derive stationary solutions, defined by the assumption that $\Psi(t,  r)$ can take the form $\Psi(t,  r) = e^{-i\omega t} \psi(r)$, where $\omega$ denotes the frequency. With this assumption, we can conveniently isolate the time-independent component of Eq. \eqref{schordingereq} using the following approach:
\ie
\frac{\partial^{2} \psi}{\partial r^{*2}} - \left[  \omega^{2} - V_{eff}(r^{*})\right]\psi = 0.\label{timeindependent}
\fe
Addressing Eq. \eqref{timeindependent} requires careful consideration of the pertinent boundary conditions. In our specific scenario, solutions meeting the necessary criteria exhibit distinct characteristics of purely ingoing behavior near the horizon
\[
    \psi^{\text{in}}(r^{*}) \sim 
\begin{cases}
    C_{l}(\omega) e^{-i\omega r^{*}} & ( r^{*}\rightarrow - \infty)\\
    A^{(-)}_{l}(\omega) e^{-i\omega r^{*}} + A^{(+)}_{l}(\omega) e^{+i\omega r^{*}} & (r^{*}\rightarrow + \infty).\label{boundaryconditions11}
\end{cases}
\]


The intricate constants, namely $C_{l}(\omega)$, $A^{(-)}_{l}(\omega)$, and $A^{(+)}_{l}(\omega)$, play a crucial role in our subsequent exploration. Broadly speaking, the frequencies $\omega_{nl}$ satisfying the condition $A^{(-)}_{l}(\omega_{nl})=0$ are termed the \textit{quasinormal} modes specific to a BH. This condition ensures that these modes manifest as a distinctly outgoing wave at spatial infinity and a purely ingoing wave at the event horizon. Within this framework, the integers $n$ and $l$ take on the roles of overtone and multipole numbers, respectively. The spectrum of \textit{quasinormal} modes unfolds through the eigenvalues derived from the solution to Eq. \eqref{timeindependent}. We employ the WKB approximation to analyse these modes by drawing upon analogies with quantum mechanics.


The WKB approximation, originally introduced by Schutz and Will \cite{1985ApJ...291L..33S}, has proven instrumental in computing \textit{quasinormal} modes within the context of particle scattering around BHs. Konoplya contributed subsequent advancements in this methodology \cite{Konoplya:2003ii, Konoplya:2004ip}. It is imperative to highlight that, for the validity of this approach, the potential must exhibit a barrier--profile, approaching constant values as $r^{*} \rightarrow \pm \infty$. By fitting the power series of the solution in the vicinity of the turning points of the maximum potential, the \textit{quasinormal} modes can be extracted \cite{Filho:2023voz}. The Konoplya formula for calculating these modes is shown below
\ie
\frac{i(\omega^{2}_{n}-V_{0})}{\sqrt{-2 V^{''}_{0}}} - \sum^{6}_{j=2} \Lambda_{j} = n + \frac{1}{2}.
\fe

Konoplya's formula for \textit{quasinormal} modes considers several crucial components in the expression above. The term $V^{''}_{0}$ signifies the second derivative of the potential evaluated at its maximum point $r_{0}$, while $\Lambda_{j}$ represents constants dependent on the effective potential and its derivatives at this maximum. Notably, recent advancements in the field have introduced a 13th-order WKB approximation proposed by Matyjasek and Opala \cite{Matyjasek:2017psv}. This development enhances the precision in calculating \textit{quasinormal} modes while contributing to the ongoing refinement of methodologies in this domain.




\begin{table}[!h]
\begin{center}
\caption{Utilizing the sixth--order WKB approximation, we investigate the quasinormal frequencies for scalar perturbations linked to various values of $\mathcal{Q}$, when $\mathcal{M}_{\alpha} =1$, $\mathcal{M}= 1$, $\lambda=10^{5}$, $\Lambda=10^{-5}$, $\alpha =1$, placing particular emphasis on instances where $l=0$.}
\label{TABI}
\begin{tabular}{c| c | c | c} 
 \hline\hline\hline 
 $\mathcal{Q}$   & $\omega_{0}$ & $\omega_{1}$ & $\omega_{2}$  \\ [0.2ex] 
 \hline 
 0.00  & 0.11046 - 0.10081$i$ & 0.08904 - 0.34446$i$ & 0.19198 - 0.47609$i$  \\ 
 
 0.10  & 0.11248 - 0.10129$i$ & 0.09125 - 0.34509$i$ & 0.19027 - 0.48145$i$  \\
 
 0.20  & 0.11461 - 0.10176$i$ & 0.09359 - 0.34573$i$  &  0.18787 - 0.48808$i$   \\
 
 0.30  & 0.11710 - 0.10205$i$ & 0.09658 - 0.34476$i$ &  0.18743 - 0.48906$i$ \\
 
 0.40 & 0.11963 - 0.10247$i$ & 0.09958 - 0.34464$i$ & 0.18460 - 0.49543$i$ \\
 
 0.50 & 0.12133 - 0.10376$i$ & 0.10074 - 0.35157$i$ & 0.17012 - 0.53405$i$  \\
 
 0.60  & 0.12601 - 0.10259$i$ & 0.10751 - 0.33846$i$ & 0.18033 - 0.49213$i$ \\
 
 0.70  & 0.12944 - 0.10167$i$ & 0.10819 - 0.33565$i$ & 0.15838 - 0.51162$i$ \\
 
 0.80  & 0.14636 - 0.08849$i$ & 0.14374 - 0.22834$i$ & 0.39365 - 0.15178$i$  \\
  
 0.90  & 0.10914 - 0.11036$i$ & 0.05450 - 0.49549$i$ & 0.03914 - 1.15009$i$  \\
 
 1.00 & 0.10914 - 0.11036$i$ & 0.05450 - 0.49549$i$ & 0.03914 - 1.15009$i$ \\
   [0.2ex] 
 \hline \hline \hline 
\end{tabular}
\end{center}
\end{table}









\begin{table}[!h]
\begin{center}
\caption{Utilizing the sixth--order WKB approximation, we investigate the quasinormal frequencies for scalar perturbations linked to various values of $\mathcal{Q}$, when $\mathcal{M}_{\alpha} =1$, $\mathcal{M}= 1$, $\lambda=10^{5}$, $\Lambda=10^{-5}$, $\alpha =1$, placing particular emphasis on instances where $l=1$.}
\label{TABII}
\begin{tabular}{c| c | c | c} 
 \hline\hline\hline 
 $\mathcal{Q}$   & $\omega_{0}$ & $\omega_{1}$ & $\omega_{2}$  \\ [0.2ex] 
 \hline 
 0.00  & 0.29289 - 0.09775$i$   & 0.26446 - 0.30650$i$  &   0.23100 - 0.54213$i$  \\ 
 
 0.10  & 0.29803 - 0.09824$i$ & 0.27016 - 0.30763$i$ & 0.23735 - 0.54322$i$ \\
 
 0.20  & 0.30358 - 0.09867$i$  & 0.27637 - 0.30858$i$  &  0.24428 - 0.54391$i$   \\
 
 0.30  & 0.30961 - 0.09904$i$ & 0.28317 - 0.30927$i$ &  0.25190 - 0.54403$i$ \\
 
 0.40 & 0.31622 - 0.09930$i$ & 0.29066 - 0.30957$i$ & 0.26029 - 0.54334$i$ \\
 
 0.50 & 0.32352 - 0.09941$i$ & 0.29897 - 0.30928$i$  & 0.26955 - 0.54143$i$  \\
 
 0.60  & 0.33167 - 0.09926$i$ & 0.30824 - 0.30807$i$ & 0.27970 - 0.53767$i$ \\
 
 0.70  & 0.34088 - 0.09869$i$ & 0.31864 - 0.30535$i$ & 0.29054 - 0.53080$i$ \\
 
 0.80 & 0.35145 - 0.09739$i$  & 0.32996 - 0.30018$i$ & 0.30034 - 0.51973$i$  \\
  
 0.90 & 0.36370 - 0.09472$i$ & 0.34109 - 0.29069$i$ & 0.30395 - 0.50308$i$ \\
 
  1.00 & 0.37740 - 0.08941$i$ & 0.34573 - 0.27790$i$ & 0.28898 - 0.50022$i$ \\
   [0.2ex] 
 \hline \hline \hline 
\end{tabular}
\end{center}
\end{table}











\begin{table}[!h]
\begin{center}
\caption{Utilizing the sixth--order WKB approximation, we investigate the quasinormal frequencies for scalar perturbations linked to various values of $\mathcal{Q}$, when $\mathcal{M}_{\alpha} =1$, $\mathcal{M}= 1$, $\lambda=10^{5}$, $\Lambda=10^{-5}$, $\alpha =1$, placing particular emphasis on instances where $l=2$.}
\label{TABIII}
\begin{tabular}{c| c | c | c} 
 \hline\hline\hline 
  $\mathcal{Q}$    & $\omega_{0}$ & $\omega_{1}$ & $\omega_{2}$  \\ [0.2ex] 
 \hline 
 0.00  & 0.48361 - 0.09676$i$ & 0.46382 - 0.29561$i$   & 0.43037 - 0.50867$i$  \\ 
 
 0.10  & 0.49202 - 0.09727$i$ & 0.47263 - 0.29702$i$ & 0.43986 - 0.51064$i$ \\
 
 0.20  & 0.50111 - 0.09773$i$ & 0.48219 - 0.29827$i$  &  0.45021 - 0.51230$i$   \\
 
 0.30  &  0.51099 - 0.09813$i$ & 0.49261 - 0.29931$i$ &  0.46153 - 0.51351$i$ \\
 
 0.40 & 0.52182 - 0.09843$i$ & 0.50406 - 0.30001$i$ & 0.47402 - 0.51407$i$ \\
 
 0.50 & 0.53379 - 0.09857$i$ & 0.51676 - 0.30020$i$ & 0.48788 - 0.51367$i$  \\
 
 0.60  & 0.54719 - 0.09847$i$ & 0.53098 - 0.29961$i$ & 0.50338 - 0.51178$i$ \\
 
 0.70  & 0.56240 - 0.09798$i$ & 0.54708 - 0.29774$i$ & 0.52077 - 0.50749$i$ \\
 
 0.80  & 0.58000 - 0.09680$i$ & 0.56549 - 0.29366$i$ & 0.54006 - 0.49915$i$  \\
  
 0.90  & 0.60093 - 0.09429$i$ & 0.58651 - 0.28541$i$ &  0.55999 - 0.48345$i$ \\
 
  1.00 & 0.62655 - 0.08874$i$ & 0.60818 - 0.26908$i$ & 0.57291 - 0.45807$i$ \\
   [0.2ex] 
 \hline \hline \hline 
\end{tabular}
\end{center}
\end{table}
The numerical values of QNMs are presented in Tables \ref{TABI}, \ref{TABII}, and \ref{TABIII}. For a fixed value of the BH mass, we obtain an increase of the real part of QNMs in all cases with the increase of electric charge. Thus, the main effect comes from the electric charge, not the Yukawa parameters. 

